Learning Human Motion from Monocular Videos via Cross-Modal Manifold Alignment

Learning 3D human motion from 2D inputs is a fundamental task in the realms of computer vision and computer graphics. Many previous methods grapple with this inherently ambiguous task by introducing motion priors into the learning process. However, these approaches face difficulties in defining the complete configurations of such priors or training a robust model. In this paper, we present the Video-to-Motion Generator (VTM), which leverages motion priors through cross-modal latent feature space alignment between 3D human motion and 2D inputs, namely videos and 2D keypoints. To reduce the complexity of modeling motion priors, we model the motion data separately for the upper and lower body parts. Additionally, we align the motion data with a scale-invariant virtual skeleton to mitigate the interference of human skeleton variations to the motion priors. Evaluated on AIST++, the VTM showcases state-of-the-art performance in reconstructing 3D human motion from monocular videos. Notably, our VTM exhibits the capabilities for generalization to unseen view angles and in-the-wild videos.

==> sec/fig/X_comp.tex <==


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{sec/fig/comparisons_supp.pdf}
  \caption{Qualitative comparisons to other SOTA methods. The green skeletons represent the ground truth poses, and the red ones represent the reconstructed poses by different methods. From top to bottom, the dance genres are House, Street Jazz, Krump, Lock, and Middle Hip-hop.}
  \label{fig:supp_comp}
\end{figure*}



==> sec/fig/X_comp_sep.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{sec/fig/comparisons_supp_sep.pdf}
  \caption{Qualitative comparisons to other SOTA methods. The green skeletons represent the ground truth poses, and the red ones represent the reconstructed poses by different methods. From top to bottom, the dance genres are House, Street Jazz, Krump, Lock, and Middle Hip-hop.}
  \label{fig:supp_comp_sep}
\end{figure*}


==> sec/fig/X_comp_wild.tex <==


\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{sec/fig/coco_wild.pdf}
  % \caption{VTM-CPN (VTM trained on the COCO-formatted 2D keyponits detected by CPN) can reconstruct motion from in-the-wild videos. The first row is the continuous frames from a wild video, and the second row illustrates the corresponding reconstructed motion by VTM-CPN.}
  \caption{VTM-CPN can reconstruct motion from in-the-wild videos. The first row is the continuous frames from a wild video, and the second row illustrates the corresponding reconstructed motion by VTM-CPN.}
  \label{fig:supp_comp_wild}
\end{figure}



==> sec/tab/11.demotab_half.tex <==
\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}
